Linearization for High-Speed Current-Steering DACs Using Neural Networks

This paper proposes a novel foreground linearization scheme for a high-speed CS-DAC. The technique leverages neural networks (NNs) to derive a LUT that maps the inverse of the DAC transfer characteristic onto the input codes. The algorithm is shown to improve conventional methods by at least 6dB in terms of intermodulation (IM) performance for frequencies up to 9GHz on a state-of-the-art 10-bit CS-DAC operating at 40.96GS/s (gigasamples-per-second) in 14nm CMOS.

==> scratch.tex <==
 as shown in Figure [], and have been employed to model CS-DACs for DPD. In this case, the system in Figure [] is described by

\begin{align} \label{hammerstein}
    y(n) = \sum_{l=0}^{L} h(l) \sum_{m=0}^P c(m) \, x(n-l)^k
\end{align}
\begin{figure}[ht]
\centering
\includegraphics[scale=0.8]{images/hammerstein_model.pdf}
\caption{Hammerstein model block diagram.}
\label{fig:hammerstein_model}
\end{figure}

Consequently, system modeling is often approached using Volterra series methods \cite{bibliography:volterra_dac}, \cite{bibliography:adc_volterra}. A complete system model involves an accurate estimate of the Volterra kernel, which is a generalization of the impulse response for linear time-invariant (LTI) systems. However, this is in general a complex task, and pruning techniques are used to reduce model complexity while still maintaining reasonable accuracy \cite{bibliography:zhu_overview_2006}. 


In addition to static errors, \ac{CS-DAC}s also exhibit dynamic errors. These errors are frequency dependent, and include any effect that disturbs the output node during code transitions. One key dynamic error to consider is switch timing mismatch between the current drivers. Ideally, all current drivers are switched simultaneously from one clock cycle to the next. However, this is not true in practice due to propagation delay mismatch in the paths leading up to the switches. Calibration for these errors is beyond the scope of this paper. 

Furthermore, the nonlinear activation function $\underbar{$h$}: \mathbb{R}^{N_H} \rightarrow \mathbb{R}^{N_H}$, is defined in the following element-wise fashion

\begin{align}
\label{eq:ReLU}
    \underbar{$h$}_i(u_i) = \max(0,u_i), \ \ i = 0, \dots, N_H-1
\end{align}

\noindent which is also known as the rectified linear unit (ReLU). The choice of ReLU is motivated by evidence that step functions can be well approximated by the difference of ReLU functions [ref], which is an attractive property given the discontinuous nature of the target function.

\section{Current-Steering DAC Background}
In this section, we introduce the CS-DAC along with its errors that contribute to nonlinear distortion. Note that covering all of them is well beyond the scope of this paper, so we only discuss those that are considered in state-of-the-art designs.

\subsection{Operation}

The basic operation of the \ac{CS-DAC} is outlined in Figure \ref{fig:high_level_cs_dac}, where the $M$-bit digital input $\left\{b_m \right\}_{m=0}^{M-1}$, clocked with period $T_s$, is converted to a differential analog output current $I_{\text{out}} = I_{\text{p}} - I_{\text{n}}$ using an array of $M$ current drivers. Each current driver contains a current source that is constructed by combining unit elements $I_\text{u}$, and the contribution of the $m^{\text{th}}$ current source to $I_{\text{out}}$ is controlled by $(b_m, \bar{b}_m) \in \left\{(1,-1), (-1,1) \right\}$. Specifically, current with weight $w_m = 2^m$ is steered to the positive branch if $b_m = 1$, and to the negative branch if $b_m = -1$. The ideal DAC output current in steady state for a particular input $\left\{b_m\right\}_{m=0}^{M-1}$ is then

\begin{align} \label{dac_out_static}
I_{\text{out}} = I_{\text{u}} \sum_{m=0}^{M-1} w_m \, b_m
\end{align}


\begin{figure}[ht]
\centering
\includegraphics[scale=0.8]{images/high_level_cs_dac.pdf}
\caption{Circuit diagram of the \ac{CS-DAC}.}
\label{fig:high_level_cs_dac}
\end{figure}

\subsection{Mismatch Errors}

In reality, the current sources shown in Figure \ref{dac_out_static} will differ from their ideal binary weights. In a CMOS process, this is typically a consequence of transistor $W/L$ and $V_T$ variation. We model this effect by augmenting the ideal weights $w_m$ in \eqref{dac_out_static} with fractional errors $\delta_m$ as follows

\begin{align} \label{dac_out_static_2}
I_{\text{out}} &= I_{\text{u}} \,  \sum_{m=0}^{M-1} w_m \left(1 + \delta_m \right) \, b_m \nonumber \\ &= I_{\text{u}} \,  \sum_{m=0}^{M-1} w_m \, b_m + I_{\text{u}} \, \sum_{m=0}^{M-1} \delta_m \, w_m \, b_m 
\end{align}

Note that \eqref{dac_out_static_2} may be interpreted as the ideal DAC output \eqref{dac_out_static} in summation with an error term. Furthermore, linearity is only impacted when there is mismatch between the $\delta_m$, since \eqref{dac_out_static_2} implies the transfer function is only adjusted by a scaling factor when $\delta_m$ are all equal. 

Typically, the LUT is derived from a Hammerstein model, which consists of a polynomial followed by a finite impulse response (FIR) filter. However, polynomials are not necessarily ideal for CS-DAC modeling, as the transfer function is prone to large discontinuities.

In contrast to polynomials, these have monotonic interpolation properties and can represent a wide array of nonlinear functions. 

A commonly used remedy for nonlinearity is Dynamic Element Matching (DEM) \cite{bibliography:DEM}. This involves randomization over the current driver cells in order to average out mismatch errors. Although generally effective, DEM incurs a noise floor penalty since the spectral shaping from this technique results in white Gaussian noise.

Another conventional technique used to enhance linearity is digital pre-distortion (DPD). In general, this involves deriving a DAC model, and then using that model to create a lookup table (LUT) that approximates the inverse of the transfer function. Such a LUT is then employed as a linearization pre-coder.

Based on Figure \ref{fig:low_freq_cw}, it is evident that system identification using a low frequency sine wave with $L=1$ results in similar performance to using random codes with $L \geq 8$. We therefore proceed with the former, which reduces the number of trainable parameters in $W_1$ by a factor of $L$. 
